Global Fits in the Supersymmetric Georgi-Machacek Model

We study a supersymmetric extension of the SM with Higgs triplets in the scalar sector. We begin with a review of the SM, particularly the Higgs mechanism. In the SM, the Higgs mechanism requires the presence of a complex Higgs doublet to break the electroweak symmetry and endow particles with a mass; this process is called Electroweak Symmetry Breaking. Although this is the simplest possibility, higher scalar representations may also contribute to the EWSB. The extent to which these higher representations contribute to EWSB is constrained by precise measurements of the $rho$ parameter. The model must predict $\rho=1$ at tree level. It is a fortuitous circumstance that simple doublet representations satisfy this requirement exactly. The underlying reason is that models with doublets satisfy an accidental custodial symmetry. Therefore, one can add any number of scalar doublets and still satisfy this experimental constraint. For higher representations, it is a bit trickier to maintain the custodial symmetry. We study in this work a supersymmetric model that incorporates triplet representations and satisfies the custodial symmetry. The non-supersymmetric Gorgi-Machacek model is one example of a custodial invariant model of SSB with Higgs triplets. However, the GM model has a fine-tuning problem beyond that of the SM. The solution to both issues is the Supersymmetric Custodial Triplet Model. The supersymmetric GM model arises as a low energy limit of the SCTM. It is this model that we study here. We make use of public code, GMCalc and HiggsTools, to perform global fits to the parameters of this model and obtain limits on model parameters at the $95%$ confidence level. For these hypothetical scalars, we identify the dominant decay channels and extract bounds on their branching ratios. We also examine the possible presence of a 95 GeV Higgs Boson in the SGM.

==> Makefile <==
# FILENAME = $(USER)_thesis
FILENAME = user_thesis

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

 LATEX = pdflatex
# LATEX = xelatex
#LATEX = lualatex

BIBTEX = bibtex
# BIBTEX = biber

default: document copy_draft

all: abstract default

abstract: abstract.pdf

abstract.pdf: latex/standalone_abstract.tex
	latexmk -$(LATEX) -logfilewarnings -halt-on-error $<
	mv standalone_abstract.pdf abstract.pdf
	rm standalone_abstract.*

figures: $(figure_list)

# Target assumes figure source is in same directory as expected figure path
figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error $(FILENAME)

document: clear_screen figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clear_screen:
	clear

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: realclean document
	mkdir submit_to_arXiv
	cp *.tex submit_to_arXiv
	cp *.bbl submit_to_arXiv/ms.bbl
	cp Makefile submit_to_arXiv
	cp -r src latex bib figures submit_to_arXiv
	if [ -d Dedman-Thesis-Latex-Template ]; then \
		mkdir submit_to_arXiv/Dedman-Thesis-Latex-Template; \
		cp Dedman-Thesis-Latex-Template/LICENSE submit_to_arXiv/Dedman-Thesis-Latex-Template/LICENSE; \
		cp -r Dedman-Thesis-Latex-Template/sty submit_to_arXiv/Dedman-Thesis-Latex-Template/sty; \
		cp -r Dedman-Thesis-Latex-Template/latex submit_to_arXiv/Dedman-Thesis-Latex-Template/latex; \
		rm submit_to_arXiv/Dedman-Thesis-Latex-Template/latex/user_commands.tex; \
		rm submit_to_arXiv/Dedman-Thesis-Latex-Template/latex/metadata.tex; \
		rm submit_to_arXiv/Dedman-Thesis-Latex-Template/latex/standalone_abstract.tex; \
	elif [ -d sty ]; then \
		cp -r sty submit_to_arXiv; \
	fi
	mv submit_to_arXiv/*_thesis.tex submit_to_arXiv/ms.tex
	# -i.bak is used for compatability across GNU and BSD/macOS sed
	# Change the FILENAME to ms while ignoring commented lines
	sed -i.bak '/^ *#/d;s/#.*//;0,/FILENAME/s/.*/FILENAME = ms/' submit_to_arXiv/Makefile
	# Remove hyperref for arXiv
	if [ -d Dedman-Thesis-Latex-Template ]; then \
		sed -i.bak '/hyperref/d' submit_to_arXiv/Dedman-Thesis-Latex-Template/latex/packages.tex; \
		sed -i.bak '/hyperref/d' submit_to_arXiv/Dedman-Thesis-Latex-Template/latex/custom_commands.tex; \
	elif [ -d sty ]; then \
		sed -i.bak '/hyperref/d' submit_to_arXiv/latex/packages.tex; \
		sed -i.bak '/hyperref/d' submit_to_arXiv/latex/custom_commands.tex; \
	fi
	find submit_to_arXiv/ -name "*.bak" -type f -delete
	# Having .tex and .pdf files of the same name will cause arXiv to delete the .pdf
	find submit_to_arXiv/figures/ -name "*.tex" -type f -delete
	# arXiv requires .bib files to be compiled to .bbl files and will remove any .bib files
	find submit_to_arXiv/ -name "*.bib" -type f -delete
	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ]; then \
		rm submit_to_arXiv.tar.gz; \
	fi


==> latex/user_commands.tex <==
% Place your own personal commands here.
% This is not a part of the base template and so will never be overwritten during updates.


==> latex/user_packages.tex <==
% Load additional packages here.
% Be careful of the loading order with respect to packages.tex as conflicts can easily arise.
% This is not a part of the base template and so will never be overwritten during updates.
\usepackage{amssymb} 

==> src/MSSM.tex <==
\begin{singlespace}
\chapter{The Minimal Supersymmetric Standard Model}\label{chapter:MSSM}
\end{singlespace}

Supersymmetry, a symmetry that relates bosons and fermions, naturally arose in string theory early in 1970s. The first consistent theory, the Minimal Supersymmetric Standard Model, was proposed in the 1980s, attempting to solve the naturalness problem, hierarchy problem and the composition of dark matter. In this dissertation, without going into to much mathematical details, we briefly review supersymmetry and the MSSM model Higgs sector\cite{baer_tata_2006}\cite{Weinberg:2000cr}\cite{djouadi2004}.

\section{Higgs Self-Energy and Naturalness Problem}

\begin{figure}[H]
 \centering
 \includegraphics[scale=0.6]{figures/higgsloop.png} \caption{\centering The Loop Contribution to Higgs Self-energy.}
 {Loop contributions to Higgs self-energy from fermions (left) and scalars (right).}
\end{figure} 

In the SM, the Yukawa interactions renders the fermion mass as $m_f=Yv/\sqrt{2}$, where $Y=\sqrt{2}m_f/v$ is the fermion-Higgs coupling. The loop integral can be written as \begin{equation}
\begin{aligned}
\Pi_{hhf}(p^2=0) & =- \int \frac{\mathrm{d}^4 k}{(2 \pi)^4} \operatorname{Tr}\left\{ \frac{i Y}{\sqrt{2}} \frac{i}{\not k-m_f} \frac{i Y}{\sqrt{2}} \frac{i}{\not k-m_f}\right\} \\
& =-2 Y^2 \int \frac{\mathrm{d}^4 k}{(2 \pi)^2}\left[\frac{k^2+m_f^2}{(k^2-m_f^2)^2}\right] .
\end{aligned}
\end{equation}
After perform the Wick rotation $k_0\rightarrow ik_0$, the integral becomes
\begin{equation}
i \int \frac{\mathrm{d}^4 k_E}{(2 \pi)^4} \frac{-k_E^2+m_f^2}{(-k_E^2-m_f^2)^2}=\frac{i}{(2 \pi)^4} \int k_E \mathrm{d} k_E \mathrm{d} \Omega \frac{(-k_E+m_f^2)}{(k_E^2+m_f^2)^2}.
\end{equation}
If we use a cutoff scale $\Lambda$, the result is 
\begin{equation}
\begin{aligned}
\Pi_{hhf}(0)&=-i\frac{Y^2}{8 \pi^2}\left[\Lambda^2-6 m_f^2 \ln\left(\frac{\Lambda}{m_f}\right)+2 m_f^2\right]+\mathcal{O}\left(\frac{1}{\Lambda^2}\right).
\end{aligned}
\end{equation}
Thus, we have a quadratic divergent contribution to the Higgs mass $\Delta m_h\sim \Lambda^2$. If we then take our cut-off energy at the scale of $\Lambda_{\text{GUT}}$ or the Planck's mass, the Higgs mass should be huge compared to the EWSB scale. This is the hierarchy problem. The discovered Higgs boson with mass around $125$GeV is very light and there is no symmetry that protects its mass from being huge. In this case we need a counterterm at the approximately the same scale as the loop contribution. This is the naturalness problem.

In the mean time, we have Higgs-scalar couplings in the SM. The contributions from the two diagrams are \begin{equation}
\begin{aligned}
\Pi_{hhS}\left(p^2\right)= &  \int \frac{d^4 k}{(2 \pi)^4}\left(i g_S\right)\left[\frac{i}{k^2-m_S^2}+\frac{i}{k^2-m_S^2}\right] \\
& +2\left(i g_S v\right)^2 \int \frac{d^4 k}{(2 \pi)^4}\left[\frac{i}{k^2-m_S^2} \frac{i}{(k+p)^2-m_S^2}\right].
\end{aligned}
\end{equation}
The contribution to $\Delta m_h$ is \begin{equation}
\begin{aligned}
\Delta m_h^2 & =\frac{ig_S}{8 \pi^2}\left[- 2\Lambda^2+4 m_S^2 \log \left(\frac{\Lambda}{m_S}\right)\right] \\
& -\frac{ig_S^2 v^2 }{8 \pi^2}\left[-1+2 \log \left(\frac{\Lambda}{m_S}\right)\right]+\mathcal{O}\left(\frac{1}{\Lambda^2}\right).
\end{aligned}
\end{equation}
Compared with the loop contributions from fermions, we find that if $m_f=m_S$ and $g_S=-Y$, the quadratic divergence is canceled out. More explicitly, if there are extra scalar particles that have opposite couplings and same mass with each SM fermions, the total radiative correction to the Higgs boson mass becomes \begin{equation}
\Delta m_h^2=\frac{Y}{4\pi^2}\left[\left(m_f^2-m_S^2\right) \log \left(\frac{\Lambda}{m_S}\right)+3 m_f^2 \log \left(\frac{m_S}{m_f}\right)\right]=0.
\end{equation}

The naturalness problem and the hierarchy problem are technically solved. That is the origination of the idea supersymmetry.

\section{The Minimal Model}

Supersymmetry is a symmetry that relates fermions and bosons. For every spin-0 and spin-1 particles in the SM, there is a spin-1/2 fermions. For every spin-1/2 fermions, there is a spin-0 scalar. In other words, the SUSY generators $\mathcal{S}$ transforms bosons into fermions and fermions into bosons: 
\begin{equation}
\mathcal{S} \mid \text{Fermion}\rangle=\mid \text{Boson}\rangle, \quad \mathcal{S}\mid\text{Boson}\rangle=\mid\text{Fermion}\rangle.
\end{equation}
When supersymmetry is exact, the bosonic fields and its fermionic superpartners have the same masses and quantum numbers, except the spin. These particles are combined into superfields. The scalar superfield contains a complex scalar field $S$ and a Majorana fermion field\footnote{A majorana fermion field is composed of one lefthanded Dirac spinor $\psi_L$ on the top and its charge conjugate $i\sigma_2\psi_L$ on the bottom.} $\psi_M$ with two components $\psi_i$. The vector super fields contains a massless gauge field $A_\mu^a$ and also a Majorana fermion field with 2 components $\lambda_a$. The canonical kinetic term in the Lagrangian is \begin{equation}
\mathcal{L}_{\text {kin }}=\sum_i\left\{\left(D_\mu S_i^*\right)\left(D^\mu S_i\right)+i \bar{\psi}_i D_\mu \gamma^\mu \psi_i\right\}+\sum_a\left\{-\frac{1}{4} F_{\mu \nu}^a F^{\mu \nu a}+\frac{i}{2} \bar{\lambda}_a D \lambda_a\right\}.
\end{equation}

For the superpotential, we need replace each field in the SM with superfields, resulting a superpartner for each SM particle. By doing that, we introduce spin-0 sfermions, such as sleptons and squarks; spin-1/2 Majorana fermions called gauginos associated with gauge bosons, and higgsinos associated with Higgs scalars, such as neutralinos and charginos. In the SM, we only have one Higgs doublet $\Phi$, which gives masses to both up-type fermions (up-type quarks), and down-type fermions (down-type quarks and electron). The down-type fermions couple to $\Phi$, whereas the up-type fermions couple to its charge conjugate $i\sigma_2\Phi^*$. When supersymmetrizing the SM Higgs sector, we need to double the number of scalar fields, one for down-type $H_1$ and one for up-type $H_2$, and couple them separately to up-type and down-type superfields in the superpotential. The is a result of the Holomorphic Principle, which states that superpotential can only depend on chiral superfields, not their complex conjugates\cite{Seiberg:1993vc}. Non-holomorphic superpotentials would make a theory non-renormalizable\cite{Bershadsky:1993ta}. 

To conserve lepton and baryon number, we impose a discrete symmetry called R-parity,
\begin{equation}
R_p=(-1)^{L+2 s+3 B},
\end{equation}
where $L$ and $B$ are the lepton number and baryon numbers and $s$ is the spin. For ordinary particles $R_p=1$ and for their superpartners $R_p=-1$. 

The most general superpotential that obey $SU(3)_C\times SU(2)_L\times U(1)_Y$ gauge invariance, renormalizablility and R-parity is \begin{equation}
W=\mu H_1 \cdot H_2+\sum_{i,j=\text{generations}}\left[Y^\ell_{ij} \bar{E}_i H_1 \cdot L_j +Y^d_{ij} \bar{D}_i H_1 \cdot Q_j +Y^u_{ij}  \bar{U}_i H_2\cdot Q \right].
\end{equation}
The superfields are summarized in Table 4.1. 
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Superfields & $SU(3)_C$& $SU(2)_L$ & $U(1)_Y$ \\
\hline $L$ & 1 & 2 & $-1$ \\
\hline $\bar{E}$ & 1 & 1 & $2$ \\
\hline $Q$ & 3 & 2 & $1/3$ \\
\hline $\bar{U}$ & $\bar{3}$ & 1 & $-4/3$ \\
\hline $\bar{D}$ & $\bar{3}$ & 1 & $2/3$\\
\hline $H_1$ & 1 & 2 & -1\\
\hline $H_2$ & 1 & 2 & 1\\
\hline
\end{tabular}
\caption[MSSM superfields and their gauge group properties.]{\centering
 MSSM superfields and their gauge group properties.}
\end{table}
In this table, $L$, $Q$ and $H_{1,2}$ are $SU(2)$ doublets. We can write them as \begin{equation}
L=\left(\begin{array}{c}
L_\nu \\
L_e
\end{array}\right), \quad Q=\left(\begin{array}{l}
Q_u \\
Q_d
\end{array}\right), \quad H_1=\left(\begin{array}{l}
H_1^0 \\
H_1^{-}
\end{array}\right), \quad H_2=\left(\begin{array}{l}
H_2^{+} \\
H_2^0
\end{array}\right).
\end{equation}
The scalar potential in the MSSM is \begin{equation}
V=V_F+V_D+V_{\text{soft}}. 
\end{equation} 
Under supersymmetry, particle and its superpartner must share the same mass value. Yet we have not observed any superpartners of the SM particles. The solution to this problem is that there is a mechanism that breaks supersymmetry. Phenomenologically, we can add a soft-supersymmetry breaking term in the Lagrangian to break SUSY explicitly. The soft SUSY-breaking term is
\begin{equation}
V_{\text {soft }}=m_1^2 H_1^{\dagger} H_1+m_2^2 H_2^{\dagger} H_2+B\mu\left(H_2 \cdot H_1+\text { h.c. }\right).
\end{equation}
The D term potential contains the quadratic interactions \begin{equation}
\begin{aligned}
V_D&=\frac{1}{2} \sum_a\left(\sum_i g_a S_i^\dagger T^a S_i\right)^2 \\
&=\frac{g_2^2}{8}\left[4\left|H_1^\dagger  H_2\right|^2-2\left(H_1^\dagger  H_2\right)\left(H_2^\dagger  H_2\right)+\left(\left|H_1\right|^2+\left|H_2\right|^2\right)\right]^2+\frac{g_1^2}{8}\left(\left|H_2\right|^2-\left|H_1\right|^2\right)^2.
\end{aligned}
\end{equation}
The F term potential is \begin{equation}
V_F=\sum_i\left|\frac{\partial W\left(\phi_j\right)}{\partial \phi_i}\right|^2=\mu^2\left(\left|H_1\right|^2+\left|H_2\right|^2\right).
\end{equation}
The full scalar potential is 
\begin{equation}
\begin{aligned}
V_H &=  \left(|\mu|^2+m_1^2\right)\left|H_1\right|^2+\left(|\mu|^2+m_2^2\right)\left|H_2\right|^2-\mu B \epsilon_{i j}\left(H_1^i H_2^j+\text { h.c. }\right) \\
& +\frac{g_2^2+g_1^2}{8}\left(\left|H_1\right|^2-\left|H_2\right|^2\right)^2+\frac{1}{2} g_2^2\left|H_1^\dagger H_2\right|^2 \\
&= M_1^2\left(\left|H_0^1\right|^2+\left|H_1^{+}\right|^2\right)+M_2^2\left(\left|H_2^0\right|^2+\left|H_2^{-}\right|^2\right)-M_3^2\left(H_1^{+} H_2^{-}-H_1^0 H_2^0+\mathrm{h.c.}\right) \\
& +\frac{g_2^2+g_1^2}{8}\left(\left|H_1^0\right|^2+\left|H_1^{+}\right|^2-\left|H_2^0\right|^2-\left|H_2^{-}\right|^2\right)^2+\frac{g_2^2}{2}\left|{H}_1^{+*} H_1^0+{H}_2^{0*} H_2^{-}\right|^2\\
&=M_1^2\left|H_0^1\right|^2+M_2^2\left|H_2^0\right|^2+M_3^2\left(H_1^0 H_2^0+\mathrm{h.c.}\right)+\frac{g_2^2+g_1^2}{8}\left(\left|H_1^0\right|^2-\left|H_2^0\right|^2\right)^2,
\end{aligned}
\end{equation}
where \begin{equation}
M_1^2=|\mu|^2+m_1^2, \quad M_2^2=|\mu|^2+m_2^2, \quad M_3^2=B_\mu.
\end{equation}
The simplifications is due to the fact that charged components do not develop vacuum expectation values. Only the neutral components develops v.e.v.s as \begin{equation}
\left\langle H_1^0\right\rangle=v_1, \quad\left\langle H_2^0\right\rangle=v_2.
\end{equation}
The tadpole conditions are \begin{equation}
\begin{aligned}
\frac{\partial V_H}{\partial H_1^0}&=2 M_1^2 v_1+2 M_3^2 v_2+\frac{1}{8}\left(g_2^2+g_1^2\right) \times 2 v_1\left(v_1^2-v_2^2\right), \\
\frac{\partial V_H}{\partial H_2^0}&=2 M_2^2 v_2-2 M_3^2 v_1+\frac{1}{8}\left(g_2^2+g_1^2\right) \times 2 v_2\left(v_2^2-v_1^2\right).
\end{aligned}
\end{equation}
We define \begin{equation}
\tan \beta=\frac{v_2}{v_1}=\frac{ \sin \beta}{\cos \beta}=\frac{s_\beta}{c_\beta}
\end{equation}
and replace $M_{1,2,3}^2$ with $B_\mu$. The physical states of MSSM Higgs sector contains two singlets and two triplets since we can decompose the Higgs fields representation as $\mathbf{2} \otimes \mathbf{2}=\mathbf{1} \oplus \mathbf{3}$. Similar to what we have done in the GM model, we decompose the fields into real and imaginary parts and shift around the v.e.vs
\begin{equation}
H_1^0\longrightarrow v_1+\frac{H_1^{0,r}+iH_1^{0,i}}{\sqrt{2}}, \quad H_2^0\longrightarrow v_2+\frac{H_2^{0,r}+iH_2^{0,i}}{\sqrt{2}}.
\end{equation}
For charged Higgs fields we have \begin{equation}
\left(H_1^{+}, H_2^{+}\right)\left(\begin{array}{cc}
m_{1}^2+\frac{1}{8} G^2\left(v_1^2-v_2^2\right)+\frac{1}{4} g_2^2 v_2^2 & B_\mu+\frac{1}{4} g_2^2 v_1 v_2 \\
B_\mu+\frac{1}{4} g_2^2 v_1 v_2 & m_{2}^2-\frac{1}{8} G^2\left(v_1^2-v_2^2\right)+\frac{1}{4} g_2^2 v_1^2
\end{array}\right)\left(\begin{array}{c}
H_1^{-} \\
H_2^{-}
\end{array}\right),
\end{equation}
where $G^2=g_1^2+g_2^2$. The matrix inside can be simplified as \begin{equation}
\mathcal{M}^2_{\text{charged}}=\left(\frac{B_\mu}{v_1 v_2}+\frac{1}{4} g_2^2\right)\left(H_1^{+}, H_2^{+}\right)\left(\begin{array}{cc}
v_2^2 & v_1 v_2 \\
v_1 v_2 & v_1^2
\end{array}\right).
\end{equation}
By diagonalizing the mass matrix we have 
\begin{equation}
\begin{split}
m_{G^{ \pm}}^2&=0, \\
m_{H^{ \pm}}^2&=\left(\frac{B_\mu}{v_1 v_2}+\frac{1}{4} g_2^2\right)\left(v_1^2+v_2^2\right)=\frac{g_2^2 v^2}{4}+\frac{B_\mu}{c_\beta s_\beta}.
\end{split}
\end{equation}
The physical states are \begin{equation}
G^{ \pm}=c_\beta H_1^{\pm}-s_\beta H_2^{\pm}, \quad H^{\pm}=s_\beta H_1^{\pm}+c_\beta H_2^{\pm}.
\end{equation}
The Goldstone boson will be absorbed by the $W^\pm$ boson, and the later acquire mass. For the pseudoscalar $(H_1^{0,i},H_2^{0,i})$, we have \begin{equation}
\mathcal{M}^2_{P}=\left(\begin{array}{cc}
m_{1 h}^2+\frac{1}{8} G^2\left(v_1^2-v_2^2\right) & B_\mu \\
B_\mu & m_{2 h}^2-\frac{1}{8} G^2\left(v_1^2-v_2^2\right)
\end{array}\right)=B_\mu\left(\begin{array}{cc}
v_2 / v_1 & 1 \\
1 & v_{1} / v_2
\end{array}\right).
\end{equation}
The masses are \begin{equation}
m_{G^0}^2=0, \quad m_A^2=\frac{B_\mu}{c_\beta s_\beta}.
\end{equation}
For the scalar $(H_1^{0,r},H_2^{0,r})$, we have
\begin{equation}
\mathcal{M}^2_{S}=\left(\begin{array}{cc}
B_\mu+\frac{1}{8} G^2\left(3 v_1^2-v_2^2\right) & -B-\frac{1}{4} G^2 v_1 v_2 \\
-B_\mu-\frac{1}{4} G^2 v_1 v_2 & B_\mu+\frac{1}{8} G^2\left(3 v_2^2-v_1^2\right)
\end{array}\right).
\end{equation}
The masses for the neutral scalars are \begin{equation}
\begin{aligned}
m_{h, H}^2 & =\frac{1}{2}\left[\mathcal{M}_{11}^2+\mathcal{M}_{22}^2 \mp \sqrt{\left(\mathcal{M}_{11}^2-\mathcal{M}_{22}^2\right)^2+4\left(\mathcal{M}_{12}^2\right)^2}\right] \\
& =\frac{1}{8} G^2 v^2+\frac{B}{\sin 2 \beta} \mp \frac{1}{8 \sin 2 \beta} \sqrt{64 B^2-16 B G^2 v^2 \cos 4 \beta \sin 2 \beta+G^4 v^4 \sin ^2 2 \beta}.
\end{aligned}
\end{equation}
The mass eigenstates $(h,H)$ can be expressed as a rotation of $\left(H_1^{0, r}, H_2^{0, r}\right)$, \begin{equation}
\left(\begin{array}{c}H \\ h\end{array}\right)=\left(\begin{array}{cc}\cos \alpha & \sin \alpha \\ -\sin \alpha & \cos \alpha\end{array}\right)\left(\begin{array}{c}H_1^{0,r} \\ H_2^{0,r}\end{array}\right).
\end{equation}
The rotation angle is obtained from \begin{equation}
\begin{aligned}
 \sin 2 \alpha&=\frac{2 \mathcal{M}_{12}^2}{\sqrt{\left(\mathcal{M}_{11}^2-\mathcal{M}_{22}^2\right)^2+4\left(\mathcal{M}_{12}^2\right)^2}}=-\frac{\left(m_H^2+m_h^2\right)}{m_H^2-m_h^2} \sin 2 \beta, \\
 \cos 2 \alpha&=\frac{\mathcal{M}_{11}^2-\mathcal{M}_{22}^2}{\sqrt{\left(\mathcal{M}_{11}^2-\mathcal{M}_{22}^2\right)^2+4\left(\mathcal{M}_{12}^2\right)^2}}=-\frac{\left(m_A^2-m_Z^2\right)}{m_H^2-m_h^2} \cos 2 \beta, \\
 \tan 2 \alpha&=\frac{2 \mathcal{M}_{12}^2}{\mathcal{M}_{11}^2-\mathcal{M}_{22}^2}=\frac{m_A^2+m_Z^2}{m_A^2-m_Z^2} \tan 2 \beta=\frac{m_h^2+m_H^2}{m_A^2-m_Z^2} \tan 2 \beta
\end{aligned}
\end{equation}
If we then impose the custodial symmetry and set \begin{equation}
v_1^2+v_2^2 \equiv v^2=\frac{1}{\sqrt{2} G_f}=\frac{2 m_Z^2}{g_1^2+g_2^2}=(246 \mathrm{GeV})^2, \quad \beta=\frac{\pi}{4}
\end{equation}
the mass spectrum becomes \begin{equation}
m_A=2 B_\mu, \quad m_{H^{ \pm}}^2=m_W^2+2B_\mu, \quad m_{h}=0,\quad m_H=m_Z^2+2B_\mu.
\end{equation}
We only have one free parameter $B_\mu$ in this custodial limit. In this limit, \begin{equation}
m_Z^2-m_W^2=\frac{1}{4} g_1^2 v^2.
\end{equation}
Custodial symmetry is also slightly broken by the hypercharge interaction $U(1)_Y$, just as in the SM. The custodial symmetry becomes exact when we take the limit $g_1\rightarrow0$ and the $W$ and $Z$ boson share the same mass.

We can also take the limit $B_\mu\rightarrow\infty$, which is the same as $m_H^2 \sim m_A^2 \sim m_{H^{ \pm}}^2\longrightarrow\infty$. Equivalently, $m^2_{H,A,H^\pm}\gg m_Z^2$. It means that all the non-SM scalar particles are decoupled from the SM ones. Thus, it is called the decoupling limit. In this limit, \begin{equation}
m_h^2=m_Z^2 \cos^2\beta, \quad |\alpha-\beta| \rightarrow \frac{\pi}{2}.
\end{equation}


\section{2HDM Model}

The 2 Higgs doublet model (2DHM) contains two complex doublet fields with opposite hypercharges
\begin{equation}
H_1=\left(\begin{array}{c}H_1^0 \\ H_1^{-}\end{array}\right), \quad H_2=\left(\begin{array}{c}
H_2^{+} \\
H_2^0
\end{array}\right)
\end{equation}
with $Y_1=1$ and $Y_2=-1$. The most general scalar potential is \begin{equation}
\begin{aligned}
V_H & =M_{11}^2 H_1^{\dagger} H_1+M_{22}^2 H_2^{\dagger} H_2 -2M_{12}^2 H_1^{\dagger} H_2 \\
& +\lambda_1\left(H_1^{\dagger} H_1\right)^2+\lambda_2\left(H_2^{\dagger} H_2\right)^2+\lambda_3 H_1^{\dagger} H_1 H_2^{\dagger} H_2+\lambda_4 H_1^{\dagger} H_2 H_2^{\dagger} H_1 \\
& +\lambda_5 H_2^{\dagger} H_1 H_2^{\dagger} H_1+\text { h.c. }.
\end{aligned}
\end{equation}
The neutral components of the two Higgs fields develop v.e.vs $v_1$ and $v_2$. We can rewrite the potential in term is $v_{1,2}$ as 
\begin{equation}
V_H=M_{11}^2 v_1^2+M_{22}^2 v_2^2-2M_{12}^2 v_1v_2+\lambda_1 v_1^4+\lambda_2 v_2^4+ (\lambda_3+\lambda_4+\lambda_5)v_1^2v_2^2
\end{equation}
Using the tadpole conditions \begin{equation}
\begin{aligned}
& \frac{\partial V_H}{\partial v_1}=2 M_{11}^2 v_1-2 M_{12}^2 v_2+4 \lambda_1 v_1^3+2\left(\lambda_3+\lambda_4+\lambda_5\right) v_1 v_2^2, \\
& \frac{\partial V_H}{\partial v_2}=2 M_{22}^2 v_2-2 M_{12}^2 v_2+4 \lambda_2 v_2^3+2\left(\lambda_3+\lambda_4+\lambda_5\right) v_1^2 v_2.
\end{aligned}
\end{equation}
We can replace $M_{11}$ and $M_{22}$ with $v_{1,2}$. The physical field consists a neutral pseudoscalar $A$ two neutral scalars $h$ and $H$ and two charged Higgs bosons $H^\pm$. The squared masses are \begin{equation}
\begin{aligned}
m_A^2&=-\left(\lambda_5-2\frac{M_{12}}{v_1 v_2}\right)\left(v_1^2+v_2^2\right),\\
m_H^{\pm}&=-\left(\frac{\lambda_4+\lambda_5}{2}-2\frac{M_{12}}{v_1 v_2}\right)\left(v_1^2+v_2^2\right),\\
m_{h,H}&=m_{h, H}^2=2M_{12}^2+\left(\lambda_1+\lambda_2\right) v_1^2 \pm \sqrt{\left(M_{12}^2+\left(\lambda_3+\lambda_4+\lambda_5\right) v_1^2\right)^2+\left(\lambda_1-\lambda_2\right)^2 v_1^4}.
\end{aligned}
\end{equation}
One of the neutral scalars can be interpreted as the SM-like 125GeV Higgs boson. 







==> src/printer_calibration.tex <==
\chapter{Printer Calibration}\label{chapter:printer_calibration}

As you may know, printers do not print your PDF file exactly.
They will scale it to match their own preset configurations and potentially add padding spaces around the edges.
There is no way to control for this as every printer is unique and there are no base standards.
The only thing a user can do is have their generated PDF file have the correct distances and then ask that the person printing their document calibrate the printer accordingly.

\printercalibration{}

\vspace{2in}
This chapter will provide printer calibrations.
All the \textcolor{red}{red lines} drawn are $1$~inch in length.
All the \textcolor{blue}{blue lines} drawn are $2$~inches in length.
These are drawn from the edge of the document in TikZ, which has good distance metrics built into it, so these distances are accurate.
Print this page and measure the margins and the length of the arrows.
If your measurements do not match those printed \textbf{you need to calibrate your printer}.
It is probable that your printer has an option that is along the lines of ``actual size'', so that might be a good starting point.
It can also help to turn on \verb|\geometry{showframe=true}| in your preamble.


==> src/results.tex <==
\begin{singlespace}
\chapter{Scan Results}\label{chapter:Results}
\end{singlespace}

